Conditional Diffusion on Web-Scale Image Pairs leads to Diverse Image Variations

Generating image variations, where a model produces variations of an input image while preserving the semantic context has gained increasing attention. Current image variation techniques involve adapting a text-to-image model to reconstruct an input image conditioned on the same image. We first demonstrate that a diffusion model trained to reconstruct an input image from frozen embeddings, can reconstruct the image with minor variations. Second, inspired by how text-to-image models learn from web-scale text-image pairs, we explore a new pretraining strategy to generate image variations using a large collection of image pairs. Our diffusion model \textit{Semantica} receives a random (encoded) image from a webpage as conditional input and denoises another noisy random image from the same webpage. We carefully examine various design choices for the image encoder, given its crucial role in extracting relevant context from the input image. Once trained, \textit{Semantica} can adaptively generate new images from a dataset by simply using images from that dataset as input. Finally, we identify limitations in standard image consistency metrics for evaluating image variations and propose alternative metrics based on few-shot generation.

==> background.tex <==
\subsection{Diffusion}

Diffusion models learn to generate examples by gradually denoising a diffusion process. For a single datapoint, their loss can be expressed as a squared error between the original datapoint and its prediction:
\begin{equation}
    \mathbb{E}_{t \sim \mathcal{U}(0, 1), \veps \sim \mathcal{N}(0, \rmI)}\big{[} w(t) || \vx - f(\vz_t) ||^2 \big{]} \text{ where } \vz_t = \alpha_t \vx + \sigma_t \veps_t
\end{equation}
It is helpful to define $\mathrm{SNR}(t) = \alpha_t^2 / \sigma_t^2$. In the case of $w(t) = \mathrm{SNR}(t)$ the loss above is equivalent to a loss in $\veps$-space, the simple loss from \citep{ho2020ddpm}. After training, the denoising model generates samples by taking small steps. Starting at $t=1$ with initial Gaussian noise and one slowly denoises for timesteps $t = 1, 1 - 1/N, \ldots$ where the number of sampling steps is $N$. Although many samplers are possible, in this paper we use the standard DDPM sampler \cite{ho2020ddpm}.


\paragraph{Architecture}
In early days, diffusion literature typically used UNets that consisted of ResNet blocks, with optional self-attention layers. More recent architecture either use full Transformers (DiT \citep{peebles2023scalable}, StableDiffusion) or transformer backbones UViTs \citep{hoogeboom2023simplediffusion}. This transformer backbone makes it especially easy to use conditioning signals in these architecture via cross-attention layers. To be precise, one can say that the denoising neural network takes in $\vz_t \in \mathbb{R}^{H \times W \times 3}, t \in \mathbb{R}, y \in \mathbb{R}^{T_y \times D_y}$. In principle it does not matter which diffusion model we use to generate images. In fact, every generative model would suffice. In practice we use the simple diffusion framework \citep{hoogeboom2023simplediffusion} because it can learn to generate high resolution images end-to-end without the need of a separate autoencoder.


